Multi-Robot Geometric Task-and-Motion Planning for Collaborative Manipulation Tasks

We address multi-robot geometric task-and-motion planning (MR-GTAMP) problems in synchronous, monotone setups. The goal of the MR-GTAMP problem is to move objects with multiple robots to goal regions in the presence of other movable objects. We focus on collaborative manipulation tasks where the robots have to adopt intelligent collaboration strategies to be successful and effective, i.e., decide which robot should move which objects to which positions, and perform collaborative actions, such as handovers. To endow robots with these collaboration capabilities, we propose to first collect occlusion and reachability information for each robot by calling motion-planning algorithms. We then propose a method that uses the collected information to build a graph structure which captures the precedence of the manipulations of different objects and supports the implementation of a mixed-integer program to guide the search for highly effective collaborative task-and-motion plans. The search process for collaborative task-and-motion plans is based on a Monte-Carlo Tree Search (MCTS) exploration strategy to achieve exploration-exploitation balance. We evaluate our framework in two challenging MR-GTAMP domains and show that it outperforms two state-of-the-art baselines with respect to the planning time, the resulting plan length and the number of objects moved. We also show that our framework can be applied to underground mining operations where a robotic arm needs to coordinate with an autonomous roof bolter. We demonstrate plan execution in two roof-bolting scenarios both in simulation and on robots.

==> pmgrs.tex <==
\begin{algorithm}
\snnote{remove for now}
\caption{PMGRS($p, O_M^G$)}\label{alg:pmgrs}
\begin{algorithmic}[1]
\WHILE {$\neg budget\_reached$}
\STATE {$queue = \text{PriorityQueue()}$}
\STATE {$\mathbf{C}^0 = \textsc{BuildCMTG}(O_M^G, p)$}
\STATE {$\mathbf{AP} = $\textsc{ApproxPlan($\mathbf{C}^0$)}}
\FOR {$AP \in \mathbf{AP}$}
\STATE {$AP.O_C = O_M$}
\STATE {$AP.\mathbf{M} = \{M \mid M \in O_M, M $ will be moved$\}$}
\STATE {$AP.V_F = \emptyset$}
\STATE {$AP.O_M^G = O_M^G$}
\STATE {$queue.add(AP, AP.length, AP.length)$}
\ENDFOR
\WHILE {$\neg queue.empty$}
\STATE {$AP = queue.pop()$}
\STATE {$a = AP.last$}
\STATE {$a.M = $ objects that will be moved}
\STATE {$k = SMPLCONT(a, AP.V_F, AP.O_C \setminus AP.\mathbf{M})$}
\STATE {$k.M = $ objects in $AP.M$ that collide with $k$}
\IF {$k$ is $\emptyset$}
\STATE {$k = SMPLCONT(a, AP.V_F, \emptyset)$}
\STATE {$k.M = $ objects in $AP.O_C$ that collide with $k$}
\ENDIF 
\IF {$k$ is $\emptyset$}
\STATE {\textbf{continue}}
\ENDIF
\STATE {$\hat{V}_F = AP.V_F + k$}
\STATE {$\hat{O}_M^G = (AP.O_M^G \setminus a.M) \cup k.M)$}
\IF {$\hat{O}_M^G = \emptyset$}
\RETURN $\hat{V}_F$
\ENDIF
\STATE {$\hat{O}_C = AP.O_C \setminus a.M$}
\STATE {$\hat{\mathbf{C}} = \textsc{BuildCMTG}(\hat{O}_M^G, p)$}
\STATE {$\hat{\mathbf{AP}} = \textsc{ApproxPlan}(\hat{\mathbf{C}})$}
\FOR {$\hat{AP} \in \hat{\mathbf{AP}}$}
\STATE {$\hat{AP}.O_C = \hat{O}_C$}
\STATE {$\hat{AP}.\mathbf{M} = \{M \mid M \in \hat{AP}.O_C, M\}$ will be moved}
\STATE {$\hat{AP}.V_F = \hat{V}_F$}
\STATE {$\hat{AP}.O_M^G = \hat{O}_M^G$}
\STATE {$queue.add(AP, \hat{AP}.V_F.length + \hat{AP}.length, \hat{AP}.length)$}
\ENDFOR 
\ENDWHILE
\RETURN {$\emptyset$}
\ENDWHILE
\RETURN {$\emptyset$}
\end{algorithmic}
\end{algorithm}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


